Optimization with Demand Oracles

We study \emph{combinatorial procurement auctions}, where a buyer with a valuation function $v$ and budget $B$ wishes to buy a set of items. Each item $i$ has a cost $c_i$ and the buyer is interested in a set $S$ that maximizes $v(S)$ subject to $\Sigma_{i\in S}c_i\leq B$. Special cases of combinatorial procurement auctions are classical problems from submodular optimization. In particular, when the costs are all equal (\emph{cardinality constraint}), a classic result by Nemhauser et al shows that the greedy algorithm provides an $\frac e {e-1}$ approximation. Motivated by many papers that utilize demand queries to elicit the preferences of agents in economic settings, we develop algorithms that guarantee improved approximation ratios in the presence of demand oracles. We are able to break the $\frac e {e-1}$ barrier: we present algorithms that use only polynomially many demand queries and have approximation ratios of $\frac 9 8+\epsilon$ for the general problem and $\frac 9 8$ for maximization subject to a cardinality constraint. We also consider the more general class of subadditive valuations. We present algorithms that obtain an approximation ratio of $2+\epsilon$ for the general problem and 2 for maximization subject to a cardinality constraint. We guarantee these approximation ratios even when the valuations are non-monotone. We show that these ratios are essentially optimal, in the sense that for any constant $\epsilon>0$, obtaining an approximation ratio of $2-\epsilon$ requires exponentially many demand queries.

==> prelim.tex <==
\section{Preliminaries}
\subsubsection*{Valuations and Problems Definition}
Let $M$ be a set of items, $|M|=m$. Let $v:2^M\rightarrow \mathbb R$ be a set function. We assume that $v(\emptyset)=0$. $v$ is \emph{monotone non-decreasing} if for each $S\subseteq T$, $v(S)\leq v(T)$.

In this paper we are mainly interested in the following two problems\footnote{We also consider some generalizations, which will be defined in the proper subsections.}: in the \emph{maximization subject to cardinality constraint} problem we are given a number $k$, and we want to find the largest value set $S$, $|S|=k$. In the \emph{maximization subject to budget constraint problem} we are given a budget $B$ and a cost $c_i$ for each item $i$. The goal is to find the largest-value set $S$, such that $\Sigma_{j\in S}c_j\leq B$. We sometimes use the name \emph{maximization subject to a knapsack constraint} for this problem.

We consider this problem under various restrictions on the valuations. We say that $v$ is \emph{submodular} if for every $S,T\subseteq M$ we have that $v(S)+v(T)\geq v(S\cup T)+v(S\cap T)$. $v$ is \emph{subadditive} if for every $S,T\subseteq M$ we have that $v(S)+v(T)\geq v(S\cup T)$. A valuation is \emph{additive} if $v(S)=\Sigma_{j\in S}v(\{j\})$. Notice that every submodular valuation is also subadditive, and every additive valuation is submodular.

Another type of valuations that we consider is fractionally subadditive (or XOS). A valuation is \emph{XOS} if there exist additive valuations $v_1,\ldots ,v_l$ such that $v(S)=\max_iv_i(S)$ (we say that $i$ is a \emph{maximizing clause} of $S$). It is known \cite {LLN01} that every XOS valuation is subadditive, and that every monotone submodular valuation is XOS, and that there are subadditive valuations that are not XOS, and XOS valuations that are not submodular.

We sometimes use the notation $v(S|T)$ to denote $v(S\cup T)-v(T)$. For the problem of maximizing a function subject to budget constraint, we sometimes use the notation $C(S)=\Sigma_{j\in S}c_j$.
\subsubsection*{Demand Queries}
Given prices $p_1,\ldots, p_m$, a \emph{demand query} returns a bundle $S$, $S\in \arg\max_Tv(T)-\Sigma_{j\in T}p_j$. The set of bundles that achieve the max is called the \emph{demand set} of the query. Our algorithms provide the guaranteed approximation ratio without making any assumption about which specific bundle is returned from the demand set. For lower bounds, as pointed out in \cite{NS05}, some unnatural tie-breaking rules may supply unrealistic information about the valuation. Therefore, as in \cite{NS05}, our lower bound assumes any tie-breaking rule that does not depend on the valuation, e.g., return the lexicographically-first bundle in the demand set.

%
%Given prices $p_1,\ldots, p_m$, a \emph{demand query} returns a bundle $S$, $S\in \arg\max_Tv(T)-\Sigma_{j\in T}p_j$. The set of bundles that achieve the max is called the \emph{demand set} of the query. Our algorithms provide the guaranteed approximation ratio without making any assumption about which specific bundle is returned from the demand set. For lower bounds, as pointed out in \cite{NS05}, some unnatural tie-breaking rules may supply unrealistic information about the valuation (e.g., when there are exponentially many bundles in the demand set, return the $t$'th bundle in the demand set, according to the lexicographic order, where $t$ is the value of the bundle of size $k$ with the highest value). Therefore, as in \cite{NS05}, our lower bound assumes any tie-breaking rule that does not depend on the valuation, e.g., return the lexicographically-first bundle in the demand set.


Another type of well-studied query is \emph{value query}: given a set $S$, return $v(S)$. It is known \cite{BN09} that a value query can be simulated by polynomially many demand queries (but exponentially many value queries may be required to simulate a single demand query). This paper concentrates in designing algorithm with polynomially many demand queries, so we freely assume that we have access to value queries.

